Blind Augmentation: Calibration-free Camera Distortion Model Estimation for Real-time Mixed-reality Consistency

Real camera footage is subject to noise, motion blur (MB) and depth of field (DoF). In some applications these might be considered distortions to be removed, but in others it is important to model them because it would be ineffective, or interfere with an aesthetic choice, to simply remove them. In augmented reality applications where virtual content is composed into a live video feed, we can model noise, MB and DoF to make the virtual content visually consistent with the video. Existing methods for this typically suffer two main limitations. First, they require a camera calibration step to relate a known calibration target to the specific cameras response. Second, existing work require methods that can be (differentiably) tuned to the calibration, such as slow and specialized neural networks. We propose a method which estimates parameters for noise, MB and DoF instantly, which allows using off-the-shelf real-time simulation methods from e.g., a game engine in compositing augmented content. Our main idea is to unlock both features by showing how to use modern computer vision methods that can remove noise, MB and DoF from the video stream, essentially providing self-calibration. This allows to auto-tune any black-box real-time noise+MB+DoF method to deliver fast and high-fidelity augmentation consistency.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> change_summary.tex <==

\onecolumn
\noindent
We thank the reviewers for their comments and address the concerns raised by them as follows.
\hrule\vspace{0.25em}
\noindent
\textbf{Q. Lack of explanation in the user study demographics and diversity [R1, R2, R3]}
\begin{itemize}
    \item We did not control for demographics as we did not expect any effect on low-level vision [Shaqiri et al. 2018]. Participants were recruited by email to authors' colleagues and the study was conducted over anonymized Google forms. The demographics consisted of students and researchers from higher education institutions in the US and Europe. In general, the subjects had research background in HCI, computer vision \& graphics, and/or psychology. We have added this statement in the final.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. User study details [R1]}
\begin{itemize}
    \item Yes, all the order of methods and scenes were randomized. 
    \item Yes, the scenes were different and we used different digital twins of animal figurines in each scene. 
    \item The stimuli used for the IDENTIFICATION task were still images shown in Fig. 11. The stimuli used for CONSISTENCY task were videos shown in the supplementary video at 03:11-03:55, which had motion blur since there was significant camera motion. 
    \item In the results for the CONSISTENCY task, it is true that the MandlEtAl method outperformed other methods except Ours that did estimate motion blur. Our hypothesis here is that users may prefer no motion blur applied to virtual objects to applying incorrect motion blur which is not consistent with the real background. Additionally, MandlEtAl still exhibited defocus blur. We note that the OkumuraEtAl++ method tended to produce exaggerated blur on virtual objects which is inconsistent. While generally offering better results, OkumuraEtAl method assumes the blur of the virtual object to be always consistent with the marker below it, which is inaccurate under many types of camera motion. 
    \item Our results of the study show that if there is blur in real scene, users can often say if there is no blur or incorrect blur on virtual objects thus making them stand out.  
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. Lack of method details [R1]}
\begin{itemize}
    \item “3 real-valued parameters (Sect. 3.1, Synthesis)” refer to the coefficients of the quadratic polynomial function $\delta(Z) = AZ^2+BZ+C$, i.e. $(A, B, C)$ as clarified in the final.This polynomial maps from depth to standard deviation of a single Gaussian kernel (we do not make use of GMMs).
    \item No, we do not fine-tune any off-the-shelf networks used. The networks are used as is for distortion removal. All network parameters are fixed as provided out-of-the-box. The parameter fitting is done on a single frame and can be performed per-frame as and when required (Sec 3.2).
    \item We came up with a heuristic to filter out homogeneous regions by taking the photometric variance of neighboring pixels in a window and thresholding. If the variance of a pixel region is less than the threshold we deem the pixel in the local region to be homogenous and discard it from the optimization.
    \item “(100 steps)” refers to the number of discrete \ac{std} values of gaussian blur kernel in the search space [0, 10] which we explore in our optimization to recover the optimal \ac{std} with which to blur each pixel based on its depth. 
    
    The code and dataset is ready and will be released following publication which will further help clarify implementation details.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. Lack of scalability evaluation [R1]}
\begin{itemize}
    \item The optimization is performed per-frame so in principle our approach can scale to any environment the neural methods are designed for. All our real scenes are captured by us and are different from the scenes on which the neural methods were trained/tested. We conclude that the methods scale well for the kind of scenes we demonstrate. We have acknowledged limitations due to neural models' performance in Sec. 5 "Limitations".
    \item We would like to clarify that the pre-trained off-the-shelf networks are only used for distortion removal (and obtaining scene geometry) while synthesis is performed by non-neural methods which do not require any training. Thus, the optimization on the input frames does not involve any neural network training.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. The model is inexact [R2]}
\begin{itemize}
    \item As addressed in our validation experiments (section 4.5), we agree that the model is inexact, but also feel there are many applications for a plausible but inexact AR system such as ours.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. Lack of explanation in the speed evaluation [R2]}
\begin{itemize}
    \item As stated in section 4.6, the sections 4.1-4.5 were obtained using a Python renderer. Section 3.1 “Speed” refers to the speed of this Python renderer for optimization (clarified in text). 
    \item In section 4.6 we demonstrate the deployment of our approach on a Meta Quest 3 headset. The speed reported in this section is the runtime of the Unity application (on the headset) which applies the distortion using our recovered parameters. The parameter estimation is done using the Python renderer by obtaining frames from the device. We show that our method recovers plausible distortion parameters to improve the augmented experience in real-time. 
    \item We believe that parameter estimation can be done online on-device too if the captured frames are exposed to developers, but since this is not the case, we had to perform the optimization offline.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. Figure 2 needs clarification [R3]}
\begin{itemize}
    \item We thank the reviewer for this observation. Indeed, the arrows to the left of minus sign should be reversed as the input to the optimization (minus sign) are the original image (orange arrows) and the synthesized image (blue arrows). 
    \item The arrows to the left of removal operation are correct, although the one to the left of synthesis operations should be reversed as well in a similar fashion. The reverse arrows were meant to signify the flow of the gradient for optimization, but we agree it is confusing. 
    \item The plus sign does represent concatenation of the parameter vectors, but since we recover each parameter separately we have removed it from the diagram for simplicity. We have revised the diagram, hoping that it is clear now.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Q. Lack of explanation about the parameter estimation [R3]}
\begin{itemize}
    \item The noise and blur removal methods we employed is a learned image-to-image approach that doesn’t directly estimate noise/blur parameters and just outputs a denoised/de-blurred image, so it was necessary in this case for us to a) assume a distortion model for synthesis and b) estimate the relevant parameters ourselves. 
    \item An interesting future exploration of our work could be investigating methods for distortion removal/synthesis which also estimates distortion parameters simultaneously, thus performing a symmetric removal followed by synthesis operation.
\end{itemize}
\hrule\vspace{0.25em}
\textbf{Minor revisions}
\begin{itemize}
    \item We have addressed all minor concerns, including fixing the typo in abstract, adding the citation provided by [R1], standardizing the method names and increasing the font size of the Figs. 4, 6, 7, 8, 10, and 11. We have also color coded the methods for clarity. 
\end{itemize}
\hrule\vspace{0.25em}

A revised version of the manuscript is provided with the added content in \add{blue color} and removed content \remove{struck out in red color}. 

\twocolumn



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

